Infinite-State Energy Games

Energy games are a well-studied class of 2-player turn-based games on a finite graph where transitions are labeled with integer vectors which represent changes in a multidimensional resource (the energy). One player tries to keep the cumulative changes non-negative in every component while the other tries to frustrate this. We consider generalized energy games played on infinite game graphs induced by pushdown automata (modelling recursion) or their subclass of one-counter automata. Our main result is that energy games are decidable in the case where the game graph is induced by a one-counter automaton and the energy is one-dimensional. On the other hand, every further generalization is undecidable: Energy games on one-counter automata with a 2-dimensional energy are undecidable, and energy games on pushdown automata are undecidable even if the energy is one-dimensional. Furthermore, we show that energy games and simulation games are inter-reducible, and thus we additionally obtain several new (un)decidability results for the problem of checking simulation preorder between pushdown automata and vector addition systems.

==> dec/reduction.tex <==
\begin{lemma}\label{lem:dec:reduction}
    For any $n$-dimensional pushdown energy game $G$
    one can (in logspace)
    construct
    \begin{enumerate}
      \item a pushdown automaton $A$,
      \item an $n$-dimensional vector addition system with states $A'$
      \item a Presburger definable function $F$ that maps a position
          $\gamma$ of the energy game to configurations $\alpha$ of $A$
          and $\beta$ of $A'$ such that Player $0$ wins from $\gamma$
          iff $\alpha\ssim \beta$.
    \end{enumerate}
    Moreover, if $G$ was a one-counter energy game,
    the constructed PDA $A$ is a one-counter automaton.

    %The fixed initial credit problem fir 1-dimensional one-counter energy games
    %is (logspace) inter-reducible with checking if
    %a configuration of a one-counter net simulates a configuration of a
    %one-counter automaton.
\end{lemma}
\begin{proof}
    todo
\end{proof}


==> pictures/3d/shorthands.tex <==
\usepackage{centernot}
%\usepackage[active,tightpage]{preview}
\usepackage{tikz}
\usepackage{pgf}
\usepackage{ifthen}


\usetikzlibrary{decorations.pathreplacing,automata,calc,positioning}
%\usepackage[latin1]{inputenc}


\newcommand{\R}{Spoiler}
\newcommand{\V}{Duplicator}

==> pictures/basic_belt.tex <==
  \def\xmax{8}
  \def\ymax{6.5}
  \def\width{8.5}
  \def\height{6}
  \def\LOx{2cm}
  \def\LOy{1cm}
  \def\pcutn{1.25}
  \def\acutn{2}
  %\def\initColour{yellow!70}
  \def\acycColour{red!40}
  \def\periodColour{green!30}
  \def\periodBorderColour{green!20!black}
  \def\initColour{blue!20}
  %\def\acycColour{red!30}
  %\def\periodColour{green!20}
  %\def\periodBorderColour{green!20!black}
\def\small{}
\def\tiny{}
\def\per{per}
\def\aper{aper}


  \begin{tikzpicture}[scale=0.4]
    \path[use as bounding box](-1.5,-0.5) rectangle ($(\width,\height) + (2.5,0.75)$);
    \tikzstyle{every node}=[font=\small]

    % Grid
    \draw[step=0.25,blue!5!white, very thin] (0,0) grid (\width,\height);
    
    % colour initial rectangle
%    \fill[\initColour] (0,0) rectangle (\LOx,\LOy);
%    \draw (\LOx,0) -- ($(\LOx,0) -(0,2pt)$) node[below] {\tiny $l_0$};
 %   \draw (0,\LOy) -- ($(0,\LOy) -(2pt,0)$) node[left] {\tiny $l_0'$};

    % -------------------------
    % draw the rest within the rectangle (0,0) to (\xmax,\ymax)
%    \begin{scope}
%      \path[clip, name path=border] (0,0) -- (0,\height) -- (\width,\height) -- (\width,0);
%      % -------------------------
%      % Points defining belt:
%      % TL, BL are points where upper and lower lines intersect y-axis.
%      % TR, BR are points where dotted lines begin
%      \coordinate (TL) at (-0.75,0);
%      \coordinate (BL) at (0.75,0);
%      \coordinate (TR) at ($(3.75,0) + (0,\acutn + 2*\pcutn)$);
%      \coordinate (BR) at ($(5.25,0) + (0,\acutn + 2*\pcutn)$);
%    
%      \path[name path=upperbeltline] (TL) -- ($(TL)!5!(TR)$);
%      \path[name path=lowerbeltline] (BL) -- ($(BL)!10!(BR)$);
%
%      % define points ATL, ATR -- Acyclic Top Left/Right
%      \path[name path=cutlevel] (0,\acutn) -- (\xmax,\acutn);
%    %  \path[name intersections={of=upperbeltline and cutlevel}];
%      \coordinate (ATL) at (intersection-1);
%    %  \path [name intersections={of=lowerbeltline and cutlevel}];
%      \coordinate (ATR) at (intersection-1);
%      
%      % define points ABL, ABR -- Acyclic Bottom Left/Right
%      \path[name path=cutlevel] (0,\LOy) -- (\xmax,\LOy);
%      \path [name intersections={of=upperbeltline and cutlevel}];
%      \coordinate (ABL) at (intersection-1);
%      \path [name intersections={of=lowerbeltline and cutlevel}];
%      \coordinate (ABR) at (intersection-1);
%    
%      \draw[dotted] (TL) -- (ABL);
%      \draw[dotted] (BL) -- (ABR);
%
%      \path[name intersections={of=lowerbeltline and border}];
%      \coordinate (MR) at (intersection-1);
%      \path[name intersections={of=upperbeltline and border}];
%      \coordinate (ML) at (intersection-2);
%
%      \begin{scope}
%          \path[clip] (TL) -- (ML) -- (MR) -- (BL);
%          % colour acyclic part red
%          \path[fill=\acycColour] (ABL) rectangle (ATR);
%
%          \path[name path=cutlevel] ($(0,\acutn + \pcutn)$) -- ($(\xmax,\acutn + \pcutn)$);
%          \path [name intersections={of=lowerbeltline and cutlevel}];
%          \coordinate (P1R) at (intersection-1);
%          \path [name intersections={of=upperbeltline and cutlevel}];
%          \coordinate (P1L) at (intersection-1);
%          
%%          \path[name path=cutlevel] ($(0,\acutn + 2*\pcutn)$) -- ($(\xmax,\acutn + 2*\pcutn)$);
%%          \path [name intersections={of=lowerbeltline and cutlevel}];
%          \coordinate (P2R) at (intersection-1);
%  %        \path [name intersections={of=upperbeltline and cutlevel}];
%          \coordinate (P2L) at (intersection-1);
%          
%%          \fill[color=\periodColour,path fading=north] (ATL) rectangle (\xmax,\ymax);
%%
%%          \path[draw,color=\periodBorderColour] (ATL) -- (ATR);
%%          \path[draw,color=\periodBorderColour] (P1L) -- (P1R);
%%          \path[draw,color=\periodBorderColour] (P2L) -- (P2R);
%      \end{scope}
%     % \draw[dotted,path fading=north](BR) -- (MR);
%      % \draw[dotted,path fading=north](TR) -- (ML);
%    \end{scope}
%    
%    
%    % belt arrows
%    \draw[->] (ABL) -- ($(ABL)!1.1!(TR)$);
%    \draw[->] (ABR) -- ($(ABR)!1.1!(BR)$);
%
%
%    % labels
%    \draw[decorate,decoration={brace,raise=0.2mm, amplitude=5pt}]
%        ($(P1R)+(4mm,0mm)$)
%        -- node[auto] {\ \per}
%        ($(ATR)+(4mm,0.5mm)$);
%
%    \draw[decorate,decoration={brace,raise=0.2mm, amplitude=5pt}]
%        ($(ATR)+(4mm,0mm)$)
%        -- node[auto] {\ \aper}
%        ($(ABR)+(4mm,0mm)$);
%
%   % \node[gray] at ($(ABL)!0.5!(ATR)$) {$A$};
% %   \node[gray] at ($(ATL)!0.5!(P1R)$) {$P_1$};
%   % \node[gray] at ($(P1L)!0.5!(P2R)$) {$P_2$};
%
%    % horizontal belt
%%    \def\alength{1cm}
%%    \def\plength{1.5cm}
%%    \def\hbheight{0.75cm}
%%    \coordinate (ATL) at ($(\LOx,\hbheight)$);
%%    \coordinate (ABL) at ($(\LOx,0)$);
%%    \coordinate (ATR) at ($(\LOx+\alength,\hbheight)$);
%%    \coordinate (ABR) at ($(\LOx+\alength,0)$);
%%    
%%    \draw[dotted] (0,\hbheight) -- (ATL);
%%    \draw[dotted] (0,0) -- (ABL);
%%    \draw[dotted] (ATR) -- (\width,\hbheight);
%%%    \begin{scope}
%%%        \path[clip] (\LOx,\hbheight) -- (\width,\hbheight) -- (\width,0) -- (\LOx,0);
%%%        % colour acyclic part red
%%%        \path[fill=\acycColour] (ABL) rectangle (ATR);
%%%
%%%        \fill[color=\periodColour,path fading=east] (ABR) rectangle (\xmax,\ymax);
%%%        \path[draw,color=\periodBorderColour] (ATR) -- (ABR);
%%%        \path[draw,color=\periodBorderColour] ($(ATR)+(\plength,0)$) -- ($(ABR)+(\plength,0)$);
%%%        \path[draw,color=\periodBorderColour] ($(ATR)+(2*\plength,0)$) -- ($(ABR)+(2*\plength,0)$);
%%%    \end{scope}
%%    \draw[->] (\LOx,\hbheight) -- ($(\LOx +5mm + \alength + 2*\plength,\hbheight)$);
%%  
%%    \draw (0,0) rectangle (\LOx,\LOy);
%%    \node[gray] at ($(0,0)!0.5!(\LOx,\LOy)$) {$L_0$};
%    
    % Axis
\draw[name path=yaxis, ->] (0,0) -- ($(0,\height)$) node[black,above] {\V };
\draw[name path=xaxis, ->] (0,0) -- ($(\width,0)$) node[black,right] {\R  };
\node at (0,0) [black, below ] {p,q};
\node at (2,2) [black, below ] {Belt};

\draw[name path=yaxis1, ->] (2,0) -- ($(\width,\height-2)$) node[black,above] {};
    \draw[name path=xaxis1, ->] (0,2) -- ($(\width-2,\height)$) node[black,right] {};
 \draw [ultra thick, draw=red, fill=red, opacity=0.3]
       (2,0) -- ($(\width,\height-2)$) -- ($(\width,0)$) -- cycle;
 \draw [ultra thick, draw=blue, fill=blue, opacity=0.3]
       (0,2) -- ($(\width-2,\height)$) -- ($(0,\height)$)  -- cycle;
      
      \node at (3,0.5) [black,right]{$\alpha$};
      
%      \draw [ultra thick, draw=green, fill=green, opacity=0.3]
%       (2,0) -- ($(\width/2+1,\height/2-1)$) -- ($(\width/2+1,0)$) -- cycle;
      
    



\end{tikzpicture}


==> pictures/border.tex <==
  \def\xmax{8}
  \def\ymax{6.5}
  \def\width{8.5}
  \def\height{6}
  \def\LOx{2cm}
  \def\LOy{1cm}
  \def\pcutn{1.25}
  \def\acutn{2}
  %\def\initColour{yellow!70}
  \def\acycColour{red!40}
  \def\periodColour{green!30}
  \def\periodBorderColour{green!20!black}
  \def\initColour{blue!20}
  %\def\acycColour{red!30}
  %\def\periodColour{green!20}
  %\def\periodBorderColour{green!20!black}
\def\small{}
\def\tiny{}
\def\per{per}
\def\aper{aper}
\def\height{10}
\def\width{10}
\def\dgreen{black!60!green}


  \begin{tikzpicture}[scale=0.4]
    \path[use as bounding box](-1.5,-0.5) rectangle ($(\width,\height) + (2.5,0.75)$);
    \tikzstyle{every node}=[font=\small]

    % Grid
    \draw[step=0.25,blue!5!white, very thin] (0,0) grid (\width,\height);
    



\draw[name path=yaxis1, \dgreen, line width=15, opacity=0.3] ($(0,\height)$) -- (0,0) -- ($(\width,0)$) node[black,above] {};
%\draw[name path=xaxis1, blue, line width=5, opacity=0.6] (0,4) -- ($(0,\height)$) node[black,right] {};
%\draw[name path=xaxis1, red, line width=5, opacity=0.6] (4,0) -- ($(\width,0)$) node[black,right] {};
\draw [fill=blue, blue, rounded corners] (-0.25,3) rectangle ($(0.25,\height)$);
\draw [fill=blue, blue] (-0.25,4) rectangle ($(0.25,\height)$);
\draw [fill=red, red, rounded corners] (4,-0.25) rectangle ($(\width, 0.25)$);
\draw [fill=red, red] (5,-0.25) rectangle ($(\width, 0.25)$);


    \node at (2,-0.5) [\dgreen, below] {border};
    \node at (8,-0.5) [red, below] {monotone part};
    \node at (-3.5,6) [blue, below] {monotone part};
    \node at (4,-0.5) [black, below] {\consts};
    \node at (-0.5,3) [black, left] {\constd};
    
    \draw[name path=yaxis, ->] (0,0) -- ($(0,\height)$) node[black,above] {\V };
\draw[name path=xaxis, ->] (0,0) -- ($(\width,0)$) node[black,right] {\R  };
\node at (0,0) [black, below ] {(s,d)};
\node at (5,4) [black, below ] {plane for states p,q};
 
      
%      \draw [ultra thick, draw=green, fill=green, opacity=0.3]
%       (2,0) -- ($(\width/2+1,\height/2-1)$) -- ($(\width/2+1,0)$) -- cycle;
      
    



\end{tikzpicture}


==> pictures/simulation.tex <==
  \def\xmax{8}
  \def\ymax{6.5}
  \def\width{8.5}
  \def\height{6}
  \def\LOx{2cm}
  \def\LOy{1cm}
  \def\pcutn{1.25}
  \def\acutn{2}
  %\def\initColour{yellow!70}
  \def\acycColour{red!40}
  \def\periodColour{green!30}
  \def\periodBorderColour{green!20!black}
  \def\initColour{blue!20}
  %\def\acycColour{red!30}
  %\def\periodColour{green!20}
  %\def\periodBorderColour{green!20!black}
\def\small{}
\def\tiny{}
\def\per{per}
\def\aper{aper}
\def\height{10}
\def\width{10}
\def\dgreen{black!60!green}


  \begin{tikzpicture}[scale=0.4]
    \path[use as bounding box](-1.5,-0.5) rectangle ($(\width,\height) + (2.5,0.75)$);
    \tikzstyle{every node}=[font=\small]

    % Grid
    \draw[step=0.25,blue!5!white, very thin] (0,0) grid (\width,\height);
    

\draw[name path=yaxis, ->] (0,0) -- ($(0,\height)$) node[black,above] {\V };
\draw[name path=xaxis, ->] (0,0) -- ($(\width,0)$) node[black,right] {\R  };
%\node at (0,0) [black, below ] {p,q};
\node at (6,6) [black, below ] {Belt};

\draw[name path=yaxis1, ->] (2,0) -- ($(\width,\height-2)$) node[black,above] {};
    \draw[name path=xaxis1, ->] (0,2) -- ($(\width-2,\height)$) node[black,right] {};
 \draw [ultra thick, draw=red, fill=red, opacity=0.3]
       (2,0) -- ($(\width,\height-2)$) -- ($(\width,0)$) -- cycle;
 \draw [ultra thick, draw=blue, fill=blue, opacity=0.3]
       (0,2) -- ($(\width-2,\height)$) -- ($(0,\height)$)  -- cycle;
      
  



%\draw[name path=yaxis1, \dgreen, line width=15, opacity=0.3] ($(0,\height)$) -- (0,0) -- ($(\width,0)$) node[black,above] {};
%\draw[name path=xaxis1, blue, line width=5, opacity=0.6] (0,4) -- ($(0,\height)$) node[black,right] {};
%\draw[name path=xaxis1, red, line width=5, opacity=0.6] (4,0) -- ($(\width,0)$) node[black,right] {};
%\draw [fill=blue, blue, rounded corners] (-0.25,3) rectangle ($(0.25,\height)$);
\draw [fill=blue, blue] (-0.25,-0.25) rectangle ($(0.25,\height)$);
%\draw [fill=red, red, rounded corners] (4,-0.25) rectangle ($(\width, 0.25)$);
\draw [fill=red, red] (0.25,-0.25) rectangle ($(\width, 0.25)$);


 %   \node at (2,-0.5) [\dgreen, below] {border};
   % \node at (8,-0.5) [red, below] {monotone part};
   % \node at (-3.5,6) [blue, below] {monotone part};
    
    \draw[name path=yaxis, ->] (0,0) -- ($(0,\height)$) node[black,above] {\V };
\draw[name path=xaxis, ->] (0,0) -- ($(\width,0)$) node[black,right] {\R  };
\node at (0,0) [black, below ] {(-1,-1)};
\node at (5,4) [black, below ] {plane for states p,q};
      
%      \draw [ultra thick, draw=green, fill=green, opacity=0.3]
%       (2,0) -- ($(\width/2+1,\height/2-1)$) -- ($(\width/2+1,0)$) -- cycle;
      
    



\end{tikzpicture}


==> pictures/solution.tex <==
  \def\xmax{8}
  \def\ymax{6.5}
  \def\width{8.5}
  \def\height{6}
  \def\LOx{2cm}
  \def\LOy{1cm}
  \def\pcutn{1.25}
  \def\acutn{2}
  %\def\initColour{yellow!70}
  \def\acycColour{red!40}
  \def\periodColour{green!30}
  \def\periodBorderColour{green!20!black}
  \def\initColour{blue!20}
  %\def\acycColour{red!30}
  %\def\periodColour{green!20}
  %\def\periodBorderColour{green!20!black}
\def\small{}
\def\tiny{}
\def\per{per}
\def\aper{aper}
\def\height{10}
\def\width{10}
\def\dgreen{black!60!green}


  \begin{tikzpicture}[scale=0.4]
    \path[use as bounding box](-1.5,-0.5) rectangle ($(\width,\height) + (2.5,0.75)$);
    \tikzstyle{every node}=[font=\small]

    % Grid
    \draw[step=0.25,blue!5!white, very thin] (0,0) grid (\width,\height);
    

% first game


\draw[name path=yaxis1, ->] (6,0) -- ($(\width,\height-6)$) node[black,above] {};
    \draw[name path=xaxis1, ->] (4,2) -- ($(\width,\height-2)$) node[black,right] {};
 \draw [ultra thick, draw=red, fill=red, opacity=0.3]
       (6,0) -- ($(\width,\height-6)$) -- ($(\width,0)$) -- cycle;







%second game




\draw[name path=yaxis1, ->] (2,3) -- ($(\width-1,\height)$) node[black,above] {};
    \draw[name path=xaxis1, ->] (0,5) -- ($(\width-5,\height)$) node[black,right] {};

 \draw [ultra thick, draw=blue, fill=blue, opacity=0.3]
       (0,5) -- ($(\width-5,\height)$) -- ($(0,\height)$)  -- cycle;





%\draw[name path=yaxis1, \dgreen, line width=15, opacity=0.3] ($(0,\height)$) -- (0,0) -- ($(\width,0)$) node[black,above] {};
%\draw[name path=xaxis1, blue, line width=5, opacity=0.6] (0,4) -- ($(0,\height)$) node[black,right] {};
%\draw[name path=xaxis1, red, line width=5, opacity=0.6] (4,0) -- ($(\width,0)$) node[black,right] {};
%\draw [fill=blue, blue, rounded corners] (-0.25,3) rectangle ($(0.25,\height)$);
\draw [fill=blue, blue] (-0.25,2.75) rectangle ($(0.25,\height)$);
\draw [fill=red, red] (4.25,-0.25) rectangle ($(\width, 0.25)$);
%\draw [fill=red, red] (5,-0.25) rectangle ($(\width, 0.25)$);



%\draw [fill=blue, blue, rounded corners, opacity=0.6] (3.75,0) rectangle ($(4.25,\height)$);
\draw [fill=blue, blue, opacity=0.6] (3.75,-0.25) rectangle ($(4.25,\height)$);
%\draw [fill=red, red, rounded corners, opacity=0.6] (0,2.75) rectangle ($(\width, 3.25)$);
\draw [fill=red, red, opacity=0.6] (0.25,2.75) rectangle ($(\width, 3.25)$);



 %   \node at (2,-0.5) [\dgreen, below] {border};
  %  \node at (8,-0.5) [red, below] {monotone part};
 %   \node at (-3.5,6) [blue, below] {monotone part};
    
    \draw[name path=yaxis, ->] (0,0) -- ($(0,\height)$) node[black,above] {\V };
\draw[name path=xaxis, ->] (0,0) -- ($(\width,0)$) node[black,right] {\R  };
\node at (0,0) [black, below ] {(s,d)};
%\node at (5,4) [black, below ] {plane for states p,q};

    \draw[name path=yaxis, ->] (4,0) -- ($(4,\height)$) node[black,above] { };
\draw[name path=xaxis, ->] (0,3) -- ($(\width,3)$) node[black,right] { };


 
      
      
%      \draw [ultra thick, draw=green, fill=green, opacity=0.3]
%       (2,0) -- ($(\width/2+1,\height/2-1)$) -- ($(\width/2+1,0)$) -- cycle;
      
    



\end{tikzpicture}


==> pictures/twogames.tex <==
  \def\xmax{8}
  \def\ymax{6.5}
  \def\width{8.5}
  \def\height{6}
  \def\LOx{2cm}
  \def\LOy{1cm}
  \def\pcutn{1.25}
  \def\acutn{2}
  %\def\initColour{yellow!70}
  \def\acycColour{red!40}
  \def\periodColour{green!30}
  \def\periodBorderColour{green!20!black}
  \def\initColour{blue!20}
  %\def\acycColour{red!30}
  %\def\periodColour{green!20}
  %\def\periodBorderColour{green!20!black}
\def\small{}
\def\tiny{}
\def\per{per}
\def\aper{aper}
\def\height{10}
\def\width{10}
\def\dgreen{black!60!green}


  \begin{tikzpicture}[scale=0.4]
    \path[use as bounding box](-1.5,-0.5) rectangle ($(\width,\height) + (2.5,0.75)$);
    \tikzstyle{every node}=[font=\small]

    % Grid
    \draw[step=0.25,blue!5!white, very thin] (0,0) grid (\width,\height);
    


%\draw[name path=yaxis1, \dgreen, line width=15, opacity=0.3] ($(0,\height)$) -- (0,0) -- ($(\width,0)$) node[black,above] {};
%\draw[name path=xaxis1, blue, line width=5, opacity=0.6] (0,4) -- ($(0,\height)$) node[black,right] {};
%\draw[name path=xaxis1, red, line width=5, opacity=0.6] (4,0) -- ($(\width,0)$) node[black,right] {};
%\draw [fill=blue, blue, rounded corners] (-0.25,3) rectangle ($(0.25,\height)$);
\draw [fill=blue, blue] (-0.25,2.75) rectangle ($(0.25,\height)$);
\draw [fill=red, red] (4.25,-0.25) rectangle ($(\width, 0.25)$);
%\draw [fill=red, red] (5,-0.25) rectangle ($(\width, 0.25)$);



%\draw [fill=blue, blue, rounded corners, opacity=0.6] (3.75,0) rectangle ($(4.25,\height)$);
\draw [fill=blue, blue, opacity=0.6] (3.75,-0.25) rectangle ($(4.25,\height)$);
%\draw [fill=red, red, rounded corners, opacity=0.6] (0,2.75) rectangle ($(\width, 3.25)$);
\draw [fill=red, red, opacity=0.6] (0.25,2.75) rectangle ($(\width, 3.25)$);



   \node at (4,-0.5) [black, below] {(\consts,d)};
   \node at (0,3) [black, left] {(s,\constd)};

    %  \node at (8,-0.5) [red, below] {monotone part};
 %   \node at (-3.5,6) [blue, below] {monotone part};
    
    \draw[name path=yaxis, ->] (0,0) -- ($(0,\height)$) node[black,above] {\V };
\draw[name path=xaxis, ->] (0,0) -- ($(\width,0)$) node[black,right] {\R  };
\node at (0,0) [black, below ] {(s,d)};
%\node at (5,4) [black, below ] {plane for states p,q};

    \draw[name path=yaxis, ->] (4,0) -- ($(4,\height)$) node[black,above] { };
\draw[name path=xaxis, ->] (0,3) -- ($(\width,3)$) node[black,right] { };


 
      
      
%      \draw [ultra thick, draw=green, fill=green, opacity=0.3]
%       (2,0) -- ($(\width/2+1,\height/2-1)$) -- ($(\width/2+1,0)$) -- cycle;
      
    



\end{tikzpicture}

